Universal Private Estimators

We present \textit{universal} estimators for the statistical mean, variance, and scale (in particular, the interquartile range) under pure differential privacy. These estimators are universal in the sense that they work on an arbitrary, unknown continuous distribution $\mathcal{P}$ over $\mathbb{R}$, while yielding strong utility guarantees except for ill-behaved $\mathcal{P}$. For certain distribution families like Gaussians or heavy-tailed distributions, we show that our universal estimators match or improve existing estimators, which are often specifically designed for the given family and under \textit{a priori} boundedness assumptions on the mean and variance of $\mathcal{P}$. This is the first time these boundedness assumptions are removed under pure differential privacy. The main technical tools in our development are instance-optimal empirical estimators for the mean and quantiles over the unbounded integer domain, which can be of independent interest.

==> Rebuttal.tex <==
We thank all reviewers for their constructive comments. Please find our responses to all reviewers' comments below.

----------------------------------------------------------
Reviewer #71A

Formal definition of "universal": You are right, our guarantees only hold for an arbitrary continuous distribution $\mathcal{P}$ over $\mathbb{R}$ (although the bound gets worse for more ill-behaved $\mathcal{P}$, i.e., with an extremely small $\varphi(\beta)$).  We will point this out more clearly, change the title, and list the discrete case (for which $\varphi(\beta)=0$) as an open problem.
 
On the first technical point: That is a good point. Yes, a Lipschitz upper bound implies a lower bound on $\varphi(\beta)$, but not vice versa.  For any $\mathcal{P}$ with a discontinuity in its pdf, its Lipschitz bound is $\infty$, but still may have a large $\varphi(\beta)$. We agree pointing out this relationship will help readers understand better.

On the second technical point: Indeed, the condition on $n$ depends on the unknown $\mathcal{P}$, so the algorithm does not know if the condition is fulfilled.  This issue actually exists in many works dealing with an unknown $\mathcal{P}$.  For example, [DL09] also imposes a condition on $n$ that depends on the unknown $\mathcal{P}$.  We will add a note to clarify it.

For all the rest comments: Thank you and we will modify the paper accordingly!

----------------------------------------------------------
Reviewer #71B

On your advice on the presentation: We admit our writing is a bit aggressive when comparing with prior work.  Per your advice, we will tone down and remove claims like  "prior work believed/claimed/overinterpreted these assumptions are necessary".  Instead, we will follow your framing: prior work focused on minimax sample complexity bounds whereas we show that one can do better on an instance-by-instance case.  In fact, the paragraph before Sec 1.1 mentioned this, but we should make it more prominent. 

On the use of SVT for removing the boundedness assumption: Yes, SVT is a standard technique, but it has not been used for removing the boundedness assumption.  Prior work used techniques like stability-based histograms, propose-test-release, and truncated distribution, but they do not work under pure-DP.  Meanwhile, there are still some difficulties when applying SVT for the problem: (1) SVT only guarantees that it will not stop too early, while here we also need to ensure that it will not stop too late. (2) Standard SVT has the log term in the error guarantee while our target is loglog, and we also provide a matching lower bound proven. (3) As mentioned in Sec 4.1, the boundedness assumption does not only mean the upper bound but also the lower bound. Prior work assume $\sigma_{max}\geq\sigma\geq \sigma_{min}$. In Sec 4.1, we give the new SVT-based solution to deal with finding a lower bound and discretizing the data. That is also where the log dependency on density is from. 

For the content of Sec 4.2: We agree an example will be helpful and we will add that. Thank you! 

On the first comment: Thank you for mentioning it. This paper is to estimate the median of a distribution with several assumptions under pure-DP. This can be used for mean estimation with a known variance and a predefined range for mean and the result is the same as [KV18]. We will add this to the related work section. 

For the second comment: Yes, they need some dependency on $\sigma_{max}/\sigma_{min}$ to give a coarse estimation for the variance. That dependency is in the $\log\log$ term (see Theorem 3.3 in that paper), which is hidden in $\tilde{O}$.

For the third comment: Yes, we will add some discussions after Theorem 1.7.

For the fourth comment: [KV18] studies how to give a private confidence interval for the mean estimation. To narrow down that interval, they also give some results for the precise estimation of the variance, where (10) is from. The result is not claimed as a theorem but in the proof: see Proposition 5.1. And yes, we miss the $1/\varepsilon$. Thank you for pointing out that. 

For the sixth comment: That is a good point. Yes, pure-DP can be achieved by using general Cauchy distribution. We will add one footnote to mention this.

For other comments: Thank you and we will modify the paper accordingly!

----------------------------------------------------------
Reviewer #71C

For high dimensions: As mentioned in Sec 1.2, using the idea of [HLY21] but replacing Gaussian mechanism with Laplace mechanism, we can extend our pure-DP estimator to the multivariate case, but it does not achieve the optimal dependency on $d$. Actually, even with boundedness assumptions, there is a $\sqrt{n}/\sqrt{d}$ gap between the state-of-art upper bound [HKM21] (accepted to STOC 22) and the lower bound under pure-DP.  We will add this discussion in Sec 1.2. 

For your advice on the presentation: We will add some sentences in Sec 1.1.1 accordingly, thank you!
